MInfoVisQA: A Multilingual Benchmark for Information-Rich Visual Question Answering

Multimodal large language models (MLLMs) excel in vision-language tasks; yet, whether they maintain consistent understanding of information-rich visuals (InfoVis) when the surface language changes remains unclear. To quantify this capability, we introduce MInfoVisQA, a parallel benchmark with 8,960 QA configurations derived from 128 seed instances across 24 languages. We construct seed-matched, language-parallel visuals and QA pairs by disentangling numerical-structural data from text and programmatically synchronizing translated labels. We evaluate 25 MLLMs under two settings: Language-Aligned QA (LQA, matching visual-text languages) and Cross-Language QA (XQA, fixed QA language with varying visual languages). The results show that aggregate accuracy masks substantial robustness gaps: two models with comparable mean LQA accuracy (80.4\%) exhibit performance spreads of 7.8 and 20.3 percentage points across languages. Moreover, all 25 models score lower with non-English visuals under fixed English QA, underscoring the need for cross-language sensitivity metrics.

==> figs/fig1_mot.tex <==
\begin{figure}[t]
  \includegraphics[width=\columnwidth]{img/img1_mot.pdf}
  \caption{Semantically equivalent information-rich visuals in different languages may elicit different interpretations from MLLMs.}
  \label{fig:fig1_mot}
\end{figure}


==> references.tex <==
%% Compiled references: original .bib files preserved unchanged.
\begin{thebibliography}{48}
\providecommand{\natexlab}[1]{#1}

\bibitem[{Ahsan et~al.(2026)Ahsan, Ahmad, Hee, Lee, and Nakov}]{tabverse}
Momina Ahsan, Sarfraz Ahmad, Ming~Shan Hee, Roy Ka-Wei Lee, and Preslav Nakov.
  2026.
\newblock Tabverse: Benchmarking cross-format table understanding in llms and
  vlms.
\newblock \emph{arXiv preprint arXiv:2606.09578}.


\bibitem[{Alam et~al.(2025)}]{rw_oasis}
Firoj Alam, Ali Ezzat Shahroor, Md. Arid Hasan, Zien Sheikh Ali, Hunzalah Hassan Bhatti, Mohamed Bayan Kmainasi, Shammur Absar Chowdhury, Basel Mousi, Fahim Dalvi, Nadir Durrani, and Natasa Milic-Frayling. 2025.
\newblock \href{https://arxiv.org/abs/2510.06371}{OASIS: A Multilingual and Multimodal Dataset for Culturally Grounded Spoken Visual QA}.
\newblock \emph{arXiv preprint arXiv:2510.06371}.

\bibitem[{Changpinyo et~al.(2023)}]{rw_maxm}
Soravit Changpinyo, Linting Xue, Michal Yarom, Ashish Thapliyal, Idan Szpektor, Julien Amelot, Xi Chen, and Radu Soricut. 2023.
\newblock \href{https://aclanthology.org/2023.findings-emnlp.176/}{MaXM: Towards Multilingual Visual Question Answering}.
\newblock \emph{Findings of the Association for Computational Linguistics: EMNLP 2023}, pages 2667--2682.


\bibitem[{Chen et~al.(2021)}]{rw_finqa}
Zhiyu Chen, Wenhu Chen, Charese Smiley, Sameena Shah, Iana Borova, Dylan Langdon, Reema Moussa, Matt Beane, Ting-Hao Huang, Bryan R. Routledge, and William Yang Wang. 2021.
\newblock \href{https://aclanthology.org/2021.emnlp-main.300/}{FinQA: A Dataset of Numerical Reasoning over Financial Data}.
\newblock \emph{Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing}, pages 3697--3711.


\bibitem[{Chen et~al.(2025)Chen, Zhao, Zeng, Huang, Zhong, and Ma}]{chartr1}
Lei Chen, Xuanle Zhao, Zhixiong Zeng, Jing Huang, Yufeng Zhong, and Lin Ma.
  2025.
\newblock Chart-r1: Chain-of-thought supervision and reinforcement for advanced
  chart reasoner.
\newblock \emph{arXiv preprint arXiv:2507.15509}.

\bibitem[{Gautam et~al.(2026)}]{rw_indotab}
Somraj Gautam, Anathapindika Dravichi, and Gaurav Harit. 2026.
\newblock \href{https://arxiv.org/abs/2604.11970}{INDOTABVQA: A Benchmark for Cross-Lingual Table Understanding in Bahasa Indonesia Documents}.
\newblock \emph{arXiv preprint arXiv:2604.11970}.


\bibitem[{Geigle et~al.(2025)Geigle, Schneider, Holtermann, Biemann, Timofte,
  Lauscher, and Glava{\v{s}}}]{geigle-etal-2025-centurio}
Gregor Geigle, Florian Schneider, Carolin Holtermann, Chris Biemann, Radu
  Timofte, Anne Lauscher, and Goran Glava{\v{s}}. 2025.
\newblock \href {https://doi.org/10.18653/v1/2025.acl-long.143} {Centurio: On
  drivers of multilingual ability of large vision-language model}.
\newblock In \emph{Proceedings of the 63rd Annual Meeting of the Association
  for Computational Linguistics (Volume 1: Long Papers)}, pages 2831--2881,
  Vienna, Austria. Association for Computational Linguistics.

\bibitem[{{Google DeepMind}(2026)}]{gemini38}
{Google DeepMind}. 2026.
\newblock {Gemini 3.8 Flash}.
\newblock \url{https://deepmind.google/models/model-cards/gemini-3-8-flash/}.
\newblock Model Card. Accessed: 2026-10-02.

\bibitem[{He et~al.(2025)}]{rw_tablelora}
Xinyi He, Yihao Liu, Mengyu Zhou, Yeye He, Haoyu Dong, Shi Han, Zejian Yuan, and Dongmei Zhang. 2025.
\newblock \href{https://arxiv.org/abs/2503.04396}{TableLoRA: Low-rank Adaptation on Table Structure Understanding for Large Language Models}.
\newblock \emph{arXiv preprint arXiv:2503.04396}.


\bibitem[{Huang et~al.(2025)Huang, Zhang, Ma, Lai, Xu, Li, Wu, Wu, and
  Liu}]{Chartsketcher}
Muye Huang, Lingling Zhang, Jie Ma, Han Lai, Fangzhi Xu, Yifei Li, Wenjun Wu,
  Yaqiang Wu, and Jun Liu. 2025.
\newblock Chartsketcher: Reasoning with multimodal feedback and reflection for
  chart understanding.
\newblock In \emph{Advances in Neural Information Processing Systems},
  volume~38.

\bibitem[{Jiang et~al.(2025)Jiang, Yu, Chen, Lu, and Zeng}]{jiang2025tabdsr}
Changjiang Jiang, Fengchang Yu, Haihua Chen, Wei Lu, and Jin Zeng. 2025.
\newblock \href {https://doi.org/10.18653/v1/2025.findings-emnlp.169} {Tabdsr:
  Decompose, sanitize, and reason for complex numerical reasoning in tabular
  data}.
\newblock In \emph{Findings of the Association for Computational Linguistics:
  EMNLP 2025}, pages 3172--3196.

\bibitem[{Jiang et~al.(2026{\natexlab{b}})Jiang, Zhao, Xin, Xie, Nakov, and
  Xie}]{jiang2026think}
Changjiang Jiang, Qiannian Zhao, Lei Xin, Jinxiang Xie, Preslav Nakov, and
  Zhuohan Xie. 2026{\natexlab{b}}.
\newblock Think with structured grounding: Perceptual reinforcement learning
  for chart and visual-tabular understanding.
\newblock \emph{arXiv preprint arXiv:2608.22429}.

\bibitem[{Kim et~al.(2024)Kim, Yim, and Song}]{kim2024tablevqa}
Yoonsik Kim, Moonbin Yim, and Ka~Yeon Song. 2024.
\newblock Tablevqa-bench: A visual question answering benchmark on multiple
  table domains.
\newblock \emph{arXiv preprint arXiv:2404.19205}.

\bibitem[{Laskar et~al.(2025)}]{rw_judges}
Md Tahmid Rahman Laskar, Mohammed Saidul Islam, Ridwan Mahbub, Ahmed Masry, Mizanur Rahman, Amran Bhuiyan, Mir Tafseer Nayeem, Shafiq Joty, Enamul Hoque, and Jimmy Huang. 2025.
\newblock \href{https://arxiv.org/abs/2505.08468}{Judging the Judges: Can Large Vision-Language Models Fairly Evaluate Chart Comprehension and Reasoning?}.
\newblock \emph{arXiv preprint arXiv:2505.08468}.


\bibitem[{Liu et~al.(2026)Liu, Lin, Wang, Gao, Li, Cai, Zhu, Zhong, Pei, Pan
  et~al.}]{chartverse}
Zheng Liu, Honglin Lin, Xiaoyang Wang, Xin Gao, Yu~Li, Mengzhang Cai, Yun Zhu,
  Zhanping Zhong, Qizhi Pei, Zhuoshi Pan, et~al. 2026.
\newblock Chartverse: Scaling chart reasoning via reliable programmatic
  synthesis from scratch.
\newblock In \emph{Proceedings of the 64th Annual Meeting of the Association
  for Computational Linguistics (Volume 1: Long Papers)}, pages 7551--7577.

\bibitem[{Lompo and Haraoui(2025)}]{visual-tableqa}
Boammani~Aser Lompo and Marc Haraoui. 2025.
\newblock Visual-tableqa: Open-domain benchmark for reasoning over table
  images.
\newblock \emph{arXiv preprint arXiv:2509.07966}.

\bibitem[{Masry et~al.(2022)Masry, Long, Tan, Joty, and
  Hoque}]{masry-etal-2022-chartqa}
Ahmed Masry, Do~Xuan Long, Jia~Qing Tan, Shafiq~R. Joty, and Enamul Hoque.
  2022.
\newblock \href {https://doi.org/10.18653/V1/2022.FINDINGS-ACL.177} {Chartqa:
  {A} benchmark for question answering about charts with visual and logical
  reasoning}.
\newblock In \emph{Findings of the Association for Computational Linguistics:
  {ACL} 2022, Dublin, Ireland, May 22-27, 2022}, volume {ACL} 2022 of
  \emph{Findings of {ACL}}, pages 2263--2279. Association for Computational
  Linguistics.

\bibitem[{Masry et~al.(2024)}]{rw_chartinstruct}
Ahmed Masry, Mehrad Shahmohammadi, Md. Rizwan Parvez, Enamul Hoque, and Shafiq Joty. 2024.
\newblock \href{https://aclanthology.org/2024.findings-acl.619/}{ChartInstruct: Instruction Tuning for Chart Comprehension and Reasoning}.
\newblock \emph{Findings of the Association for Computational Linguistics: ACL 2024}, pages 10387--10409.


\bibitem[{Masry et~al.(2025a)Masry, Islam, Ahmed, Bajaj, Kabir, Kartha, Laskar,
  Rahman, Rahman, Shahmohammadi, Thakkar, Parvez, Hoque, and
  Joty}]{masry-etal-2025-chartqapro}
Ahmed Masry, Mohammed~Saidul Islam, Mahir Ahmed, Aayush Bajaj, Firoz Kabir,
  Aaryaman Kartha, Md. Tahmid~Rahman Laskar, Mizanur Rahman, Shadikur Rahman,
  Mehrad Shahmohammadi, Megh Thakkar, Md.~Rizwan Parvez, Enamul Hoque, and
  Shafiq Joty. 2025a.
\newblock \href {https://doi.org/10.18653/V1/2025a.FINDINGS-ACL.978}
  {Chartqapro: {A} more diverse and challenging benchmark for chart question
  answering}.
\newblock In \emph{Findings of the Association for Computational Linguistics,
  {ACL} 2025, Vienna, Austria, July 27 - August 1, 2025}, volume {ACL} 2025 of
  \emph{Findings of {ACL}}, pages 19123--19151. Association for Computational
  Linguistics.

\bibitem[{Masry et~al.(2025b)}]{rw_bigcharts}
Ahmed Masry, Abhay Puri, Masoud Hashemi, Juan A. Rodriguez, Megh Thakkar, Khyati Mahajan, Vikas Yadav, Sathwik Tejaswi Madhusudhan, Alexandre Pich{\'{e}}, Dzmitry Bahdanau, Christopher Pal, David Vazquez, Enamul Hoque, Perouz Taslakian, Sai Rajeswar, and Spandana Gella. 2025b.
\newblock \href{https://arxiv.org/abs/2508.09804}{BigCharts-R1: Enhanced Chart Reasoning with Visual Reinforcement Finetuning}.
\newblock \emph{arXiv preprint arXiv:2508.09804}.


\bibitem[{{MiniMax}(2026)}]{minimaxm3}
{MiniMax}. 2026.
\newblock {MiniMax M3}: Frontier coding, 1m context, native multimodality---all
  in one model.
\newblock \url{https://www.minimax.io/blog/minimax-m3/}.
\newblock Accessed: 2026-10-02.

\bibitem[{Nan et~al.(2022)}]{rw_fetaqa}
Linyong Nan, Chiachun Hsieh, Ziming Mao, Xi Victoria Lin, Neha Verma, Rui Zhang, Wojciech Kry{\'{s}}ci{\'{n}}ski, Hailey Schoelkopf, Riley Kong, Xiangru Tang, Mutethia Mutuma, Ben Rosand, Isabel Trindade, Renusree Bandaru, Jacob Cunningham, Caiming Xiong, and Dragomir Radev. 2022.
\newblock \href{https://aclanthology.org/2022.tacl-1.3/}{FeTaQA: Free-form Table Question Answering}.
\newblock \emph{Transactions of the Association for Computational Linguistics}, pages 35--49.


\bibitem[{{OpenAI}(2026{\natexlab{a}})}]{gpt56}
{OpenAI}. 2026{\natexlab{a}}.
\newblock {GPT-5.6: Frontier Intelligence That Scales with Your Ambition}.
\newblock \url{https://openai.com/index/gpt-5-6/}.
\newblock Accessed: 2026-10-02.

\bibitem[{{OpenAI}(2026{\natexlab{b}})}]{gpt6}
{OpenAI}. 2026{\natexlab{b}}.
\newblock {GPT-6 Astra: A New Generation of Intelligence}.
\newblock \url{https://openai.com/index/gpt-6-astra/}.
\newblock Accessed: 2026-10-02.

\bibitem[{{OpenAI}(2026{\natexlab{c}})}]{gpt55}
{OpenAI}. 2026{\natexlab{c}}.
\newblock {Introducing GPT‑5.5}.
\newblock \url{https://openai.com/index/introducing-gpt-5-5/}.
\newblock Accessed: 2026-10-02.

\bibitem[{Pfeiffer et~al.(2022)}]{rw_xgqa}
Jonas Pfeiffer, Gregor Geigle, Aishwarya Kamath, Jan-Martin O. Steitz, Stefan Roth, Ivan Vuli{\'{c}}, and Iryna Gurevych. 2022.
\newblock \href{https://aclanthology.org/2022.findings-acl.196/}{xGQA: Cross-Lingual Visual Question Answering}.
\newblock \emph{Findings of the Association for Computational Linguistics: ACL 2022}, pages 2497--2511.


\bibitem[{{Qwen Team}(2026)}]{qwen38}
{Qwen Team}. 2026.
\newblock \href {https://qwen.ai/blog?id=qwen3.8} {Qwen3.8-max: A new bar for
  coding and cowork}.

\bibitem[{Romero et~al.(2024)}]{rw_cvqa}
David Romero, Chenyang Lyu, Haryo Akbarianto Wibowo, Teresa Lynn, Injy Hamed, Aditya Nanda Kishore, Aishik Mandal, Alina Dragonetti, Artem Abzaliev, Atnafu Lambebo Tonja, Bontu Fufa Balcha, Chenxi Whitehouse, Christian Salamea, Dan John Velasco, David Ifeoluwa Adelani, David Le Meur, Emilio Villa-Cueva, Fajri Koto, Fauzan Farooqui, and 57 others. 2024.
\newblock \href{https://arxiv.org/abs/2406.05967}{CVQA: Culturally-diverse Multilingual Visual Question Answering Benchmark}.
\newblock \emph{arXiv preprint arXiv:2406.05967}.


\bibitem[{Shahroor et~al.(2026)}]{rw_memelens}
Ali Ezzat Shahroor, Mohamed Bayan Kmainasi, Abul Hasnat, Dimitar Dimitrov, Giovanni Da San Martino, Preslav Nakov, and Firoj Alam. 2026.
\newblock \href{https://arxiv.org/abs/2601.12539}{MemeLens: Multilingual Multitask VLMs for Memes}.
\newblock \emph{arXiv preprint arXiv:2601.12539}.


\bibitem[{Shu et~al.(2026)}]{rw_m3tqa}
Daixin Shu, Jian Yang, Zhenhe Wu, Xianjie Wu, Xianfu Cheng, Xiangyuan Guan, Yanghai Wang, Pengfei Wu, Tingyang Yang, Hualei Zhu, Wei Zhang, Ge Zhang, Jiaheng Liu, and Zhoujun Li. 2026.
\newblock \href{https://aclanthology.org/2026.findings-acl.1134/}{M3TQA: Massively Multilingual Multitask Table Question Answering}.
\newblock \emph{Findings of the Association for Computational Linguistics: ACL 2026}, pages 22578--22602.


\bibitem[{Tang et~al.(2025{\natexlab{a}})Tang, Liu, Ye, Lu, Wei, Wang, Lin,
  Feng, Zhao, Wang, Liu, Liu, Bai, and Huang}]{tang-etal-2025-mtvqa}
Jingqun Tang, Qi~Liu, Yongjie Ye, Jinghui Lu, Shu Wei, An-Lan Wang, Chunhui
  Lin, Hao Feng, Zhen Zhao, Yanjie Wang, Yuliang Liu, Hao Liu, Xiang Bai, and
  Can Huang. 2025{\natexlab{a}}.
\newblock \href {https://doi.org/10.18653/v1/2025.findings-acl.404} {{MTVQA}:
  Benchmarking multilingual text-centric visual question answering}.
\newblock In \emph{Findings of the Association for Computational Linguistics:
  ACL 2025}, pages 7748--7763, Vienna, Austria. Association for Computational
  Linguistics.

\bibitem[{Tang et~al.(2025{\natexlab{b}})Tang, Kim, Zhao, Lake, Ding, Yin,
  Singhal, Wadhwa, Liu, Sprague, Namuduri, Hu, Rodriguez, Peng, and
  Durrett}]{chartmuseum}
Liyan Tang, Grace Kim, Xinyu Zhao, Thom Lake, Wenxuan Ding, Fangcong Yin,
  Prasann Singhal, Manya Wadhwa, Zeyu~Leo Liu, Zayne Sprague, Ramya Namuduri,
  Bodun Hu, Juan~Diego Rodriguez, Puyuan Peng, and Greg Durrett.
  2025{\natexlab{b}}.
\newblock \href
  {http://papers.nips.cc/paper\_files/paper/2025/hash/ca20efa9cf3703186d91424cf4876f8b-Abstract-Datasets\_and\_Benchmarks\_Track.html}
  {Chartmuseum: Testing visual reasoning capabilities of large vision-language
  models}.
\newblock In \emph{Advances in Neural Information Processing Systems 38: Annual
  Conference on Neural Information Processing Systems 2025, NeurIPS 2025, San
  Diego, CA, USA, December 2-7, 2025 / Mexico City, Mexico, November 30 -
  December 5, 2025}.

\bibitem[{Team(2026{\natexlab{b}})}]{qwen35}
Qwen Team. 2026{\natexlab{b}}.
\newblock \href {https://qwen.ai/blog?id=qwen3.5} {Qwen3.5: Towards native
  multimodal agents}.

\bibitem[{Team et~al.(2026{\natexlab{a}})Team, Huang, Zhang, Fu, Jiang, Qu,
  Zhang, Cui, Zhang, Xie et~al.}]{team2026polyocr}
GuangJian Team, Kaili Huang, Yongshuo Zhang, Bingtao Fu, Changjiang Jiang,
  Chenfan Qu, Chenfeng Zhang, Fangming Cui, Gaoyang Zhang, Jiangwei Xie, et~al.
  2026{\natexlab{a}}.
\newblock Polyocr-venus: Unified ocr foundation models for text-centric visual
  intelligence.
\newblock \emph{arXiv preprint arXiv:2609.37712}.

\bibitem[{Team et~al.(2026{\natexlab{b}})Team, Bai, Bai, Bao, Cai, Cai, Cao,
  Cao, Chai, Charles et~al.}]{team2026kimi}
Kimi Team, Tongtong Bai, Yifan Bai, Yiping Bao, Jianfeng Cai, Xinyuan Cai,
  Peizhou Cao, Yuxuan Cao, Ziwei Chai, Y~Charles, et~al. 2026{\natexlab{b}}.
\newblock Kimi k3: Open frontier intelligence.
\newblock \emph{arXiv preprint arXiv:2607.24653}.

\bibitem[{Wang et~al.(2024)Wang, Xia, He, Chen, Liu, Zhu, Liang, Wu, Liu,
  Malladi, Chevalier, Arora, and Chen}]{charxiv}
Zirui Wang, Mengzhou Xia, Luxi He, Howard Chen, Yitao Liu, Richard Zhu, Kaiqu
  Liang, Xindi Wu, Haotian Liu, Sadhika Malladi, Alexis Chevalier, Sanjeev
  Arora, and Danqi Chen. 2024.
\newblock \href
  {http://papers.nips.cc/paper\_files/paper/2024/hash/cdf6f8e9fd9aeaf79b6024caec24f15b-Abstract-Datasets\_and\_Benchmarks\_Track.html}
  {Charxiv: Charting gaps in realistic chart understanding in multimodal llms}.
\newblock In \emph{Advances in Neural Information Processing Systems 37: Annual
  Conference on Neural Information Processing Systems 2024, NeurIPS 2024,
  Vancouver, BC, Canada, December 10 - 15, 2024}.

\bibitem[{Wei et~al.(2026)Wei, He, Lan, Dong, Cai, Li, Zhu, Wang, Kong, Wang
  et~al.}]{wei2026zooming}
Lai Wei, Liangbo He, Jun Lan, Lingzhong Dong, Yutong Cai, Siyuan Li, Huijia
  Zhu, Weiqiang Wang, Linghe Kong, Yue Wang, et~al. 2026.
\newblock Zooming without zooming: Region-to-image distillation for
  fine-grained multimodal perception.
\newblock \emph{arXiv preprint arXiv:2602.11858}.

\bibitem[{Xie et~al.(2026)Xie, Orel, Thareja, Sahnan, Madmoun, Zhang, Banerjee,
  Georgiev, Peng, Qian, Huang, Su, Singh, Xing, Elbadry, Xu, Li, Koto, Koychev,
  Chakraborty, Wang, Lahlou, Stoyanov, Ananiadou, and
  Nakov}]{xie-etal-2026-finchain}
Zhuohan Xie, Daniil Orel, Rushil Thareja, Dhruv Sahnan, Hachem Madmoun, Fan
  Zhang, Debopriyo Banerjee, Georgi~Nenkov Georgiev, Xueqing Peng, Lingfei
  Qian, Jimin Huang, Jinyan Su, Aaryamonvikram Singh, Rui Xing, Rania Elbadry,
  Chen Xu, Haonan Li, Fajri Koto, Ivan Koychev, and 6 others. 2026.
\newblock \href {https://doi.org/10.18653/v1/2026.acl-long.662} {{F}in{C}hain:
  A symbolic benchmark for verifiable chain-of-thought financial reasoning}.
\newblock In \emph{Proceedings of the 64th Annual Meeting of the {A}ssociation
  for {C}omputational {L}inguistics (Volume 1: Long Papers)}, pages
  14529--14553, San Diego, California, United States. Association for
  Computational Linguistics.

\bibitem[{Xing et~al.(2025)Xing, He, Zhou, Dong, Han, Chen, Zhang, Chaudhuri,
  and Jagadish}]{xing2025mmtu}
Junjie Xing, Yeye He, Mengyu Zhou, Haoyu Dong, Shi Han, Lingjiao Chen, Dongmei
  Zhang, Surajit Chaudhuri, and H.~V. Jagadish. 2025.
\newblock \href
  {http://papers.nips.cc/paper\_files/paper/2025/hash/63b3985ad1dade84a34d581590e5f608-Abstract-Datasets\_and\_Benchmarks\_Track.html}
  {{MMTU:} {A} massive multi-task table understanding and reasoning benchmark}.
\newblock In \emph{Advances in Neural Information Processing Systems 38: Annual
  Conference on Neural Information Processing Systems 2025, NeurIPS 2025, San
  Diego, CA, USA, December 2-7, 2025 / Mexico City, Mexico, November 30 -
  December 5, 2025}.

\bibitem[{Xu et~al.(2026)}]{rw_modora}
Bangrui Xu, Qihang Yao, Zirui Tang, Xuanhe Zhou, Yeye He, Shihan Yu, Qianqian Xu, Bin Wang, Guoliang Li, Conghui He, and Fan Wu. 2026.
\newblock \href{https://arxiv.org/abs/2602.23061}{MoDora: Tree-Based Semi-Structured Document Analysis System}.
\newblock \emph{arXiv preprint arXiv:2602.23061}.


\bibitem[{Xu et~al.(2026{\natexlab{a}})Xu, Li, Lin, Xue, Xian, Xu, Wu, Zhang,
  Deng, Yu et~al.}]{xu2026deepseek}
Anyi Xu, B~Li, Bangcai Lin, Bing Xue, BingCheng Xian, Bingzheng Xu, Bochao Wu,
  Bowei Zhang, Boyi Deng, CC~Yu, et~al. 2026{\natexlab{a}}.
\newblock Deepseek-v4.1-flash: Pushing the limits of kv cache compression.
\newblock \emph{arXiv preprint arXiv:2609.19969}.

\bibitem[{Xu et~al.(2026{\natexlab{b}})Xu, Chen, Zhang, Yue, Ma, Wang, and
  Jin}]{polychartqa}
Yichen Xu, Liangyu Chen, Liang Zhang, Zihao Yue, Jianzhe Ma, Wenxuan Wang, and
  Qin Jin. 2026{\natexlab{b}}.
\newblock \href {https://doi.org/10.18653/v1/2026.acl-long.2043}
  {{POLYCHARTQA}: Benchmarking large vision-language models with multilingual
  chart question answering}.
\newblock In \emph{Proceedings of the 64th Annual Meeting of the {A}ssociation
  for {C}omputational {L}inguistics (Volume 1: Long Papers)}, pages
  44154--44186, San Diego, California, United States. Association for
  Computational Linguistics.

\bibitem[{Yuan et~al.(2025)Yuan, Zhang, Li, Cai, Yao, Chen, Wang, Hou, Chen,
  Jiang, and Li}]{cite_segui}
Xinbin Yuan, Jian Zhang, Kaixin Li, Zhuoxuan Cai, Lujian Yao, Jie Chen, Enguang
  Wang, Qibin Hou, Jinwei Chen, Peng-Tao Jiang, and Bo~Li. 2025.
\newblock \href
  {https://proceedings.neurips.cc/paper_files/paper/2025/file/b95c7e24501f5d1dddbc5e8526cda7ae-Paper-Conference.pdf}
  {Se-gui: Enhancing visual grounding for gui agents via self-evolutionary
  reinforcement learning}.
\newblock In \emph{Advances in Neural Information Processing Systems},
  volume~38, pages 127658--127679. Curran Associates, Inc.

\bibitem[{Yuan et~al.(2026)Yuan, Lou, Yu, Lin, Sun, Han, and
  Lu}]{yuan2026vision}
Qianhao Yuan, Jie Lou, Xing Yu, Hongyu Lin, Le~Sun, Xianpei Han, and Yaojie Lu.
  2026.
\newblock Vision-opd: Learning to see fine details for multimodal llms via
  on-policy self-distillation.
\newblock \emph{arXiv preprint arXiv:2605.18740}.

\bibitem[{Yu et~al.(2025)Yu, Feng, Li, Liao, Yu, Feng, Zhong, Chen, Hu, Wu
  et~al.}]{xtvqa}
Xinmiao Yu, Xiaocheng Feng, Yun Li, Minghui Liao, Ya-Qi Yu, Xiachong Feng,
  Weihong Zhong, Ruihan Chen, Mengkang Hu, Jihao Wu, et~al. 2025.
\newblock Cross-lingual text-rich visual comprehension: An information theory
  perspective.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, volume~39, pages 9680--9688.

\bibitem[{Zhang et~al.(2025)}]{rw_multitat}
Xuanliang Zhang, Dingzirui Wang, Keyan Xu, Qingfu Zhu, and Wanxiang Che. 2025.
\newblock \href{https://aclanthology.org/2025.findings-emnlp.33/}{MULTITAT: Benchmarking Multilingual Table-and-Text Question Answering}.
\newblock \emph{Findings of the Association for Computational Linguistics: EMNLP 2025}, pages 626--647.


\bibitem[{Zhou et~al.(2026)Zhou, Zhao, Wu, Dong, Wang, Liu, Liu, Xu, Wang, Luo
  et~al.}]{zhou2026incentivizing}
Jiang Zhou, Xiaohu Zhao, Xinwei Wu, Tianyu Dong, Hao Wang, Yangyang Liu, Heng
  Liu, Linlong Xu, Longyue Wang, Weihua Luo, et~al. 2026.
\newblock Incentivizing parametric knowledge via reinforcement learning with
  verifiable rewards for cross-cultural entity translation.
\newblock In \emph{Proceedings of the 64th Annual Meeting of the Association
  for Computational Linguistics (Volume 1: Long Papers)}, pages 5616--5638.

\bibitem[{Zhu et~al.(2021)}]{rw_tatqa}
Fengbin Zhu, Wenqiang Lei, Youcheng Huang, Chao Wang, Shuo Zhang, Jiancheng Lv, Fuli Feng, and Tat-Seng Chua. 2021.
\newblock \href{https://aclanthology.org/2021.acl-long.254/}{TAT-QA: A Question Answering Benchmark on a Hybrid of Tabular and Textual Content in Finance}.
\newblock \emph{Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)}, pages 3277--3287.

\end{thebibliography}

